Learning Task Constraints from Demonstration for Hybrid Force/Position Control

We present a novel method for learning hybrid force/position control from demonstration. We learn a dynamic constraint frame aligned to the direction of desired force using Cartesian Dynamic Movement Primitives. In contrast to approaches that utilize a fixed constraint frame, our approach easily accommodates tasks with rapidly changing task constraints over time. We activate only one degree of freedom for force control at any given time, ensuring motion is always possible orthogonal to the direction of desired force. Since we utilize demonstrated forces to learn the constraint frame, we are able to compensate for forces not detected by methods that learn only from demonstrated kinematic motion, such as frictional forces between the end-effector and contact surface. We additionally propose novel extensions to the Dynamic Movement Primitive framework that encourage robust transition from free-space motion to in-contact motion in spite of environment uncertainty. We incorporate force feedback and a dynamically shifting goal to reduce forces applied to the environment and retain stable contact while enabling force control. Our methods exhibit low impact forces on contact and low steady-state tracking error.

==> problem_statement.tex <==
\vspace{-2pt}
\section{Problem Statement and Approach}
\vspace{-2pt}
\label{sec:problem_definition}

We consider the scenario where a robot needs to move through free-space, make
contact with a surface, and perform a motion along the surface while applying a
desired force. We highlight two challenges that arise in this task setting.

First, the surface may not be exactly at the anticipated position (e.g. table
height, distance to wall), either from perceptual error or from the surface
distance changing slightly. Large impact forces can result if the surface is
closer than expected and force control is not enabled at contact, or if the
surface is farther than expected and integral terms in force control wind
up~\cite{wilfinger1992comparison}. In the latter case, stable contact can be
difficult to achieve, particularly when making contact with a stiff
surface~\cite{mandal1993experimental}. We propose to address this first
challenge with novel extensions to the DMP framework that allow for robustly
making stable contact and transitioning into constrained motion. Our extensions
incorporate force feedback and contact awareness to reduce contact forces and
gradually transition into tracking desired forces. To accommodate making contact
with surfaces at different positions than anticipated we define a dynamically
changing goal that transitions as a function of the robot's contact with the
environment.

Second, the subtask of performing a motion along a surface while applying a
desired force requires a control law that can track both force and position
simultaneously. Hybrid force/position control is a popular choice since it
allows two disjoint task space control objectives to be tracked without
conflicting control priorities. However, this control paradigm inherently
requires the choice of a constraint frame and the selection of which dimensions
of the constraint frame are devoted to force and position control. Devoting more
dimensions to force control leaves fewer dimensions available to position
control. Thus, a poor choice of constraint frame can impede the robot's ability
to meet the force/position control objectives. For tasks with rapidly changing
force constraints, this choice becomes infeasible. We address this second
challenge by using Cartesian Dynamic Movement Primitives (CDMPs) to learn a
dynamic constraint frame aligned to desired forces for which force constraints
are trivially specified. We embed the learned constraint frame in an operational
space hybrid force/position control law to simultaneously meet position and
force control objectives without the burden of manually defining the appropriate
constraint frame and task constraints.

